Studies of Vector Boson Scattering And Triboson Production with DELPHES Parametrized Fast Simulation for Snowmass 2013

Multiboson production provides a unique way to probe Electroweak Symmetry Breaking (EWSB) and physics beyond the Standard Model (SM). With the discovery of the Higgs boson, the default model is that EWSB occurs according to the Higgs mechanism. Deviations from the SM in Higgs and gauge boson properties due to new physics at a higher energy scale can be parameterized by higher-dimension operators in an Effective Field Theory (EFT). We present sensitivity studies for dimension-6 and dimension-8 operators in an EFT by looking for anomalous vector boson scattering and triboson production, at proton-proton colliders with center-of-mass energies of 14 TeV, 33 TeV and 100 TeV, respectively.

==> EWdim6VVV.tex <==
\section{Tribosons with dimension 6 operators}

In addition to the dimension 8 operators discussed in Sec.~\ref{WWW}, we have also considered dimension 6 operators.  All processes studied were decayed fully leptonically using the same generator and event selection as for the dimension 8 operators in Sec.~\ref{WWW}. Before choosing an operator to study in more detail, we completed a scan of the cross-section values for different operators, using a common center-of-mass energy of 14~\TeV and common coupling strength of $5^{-2}$ TeV.  This scan is shown in Table~\ref{tab:dim6scan}.  The largest deviation from the standard model cross-section is for the Cwww operator for both $WWW$ and $WZZ$.  Of these two, we choose to study $WWW$ because the overall cross-section is larger, and the backgrounds are better understood due to our earlier study of the dimension 8 operators with $WWW$.

\begin{table}[htdp]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Coupling & $WWW$ & $WWZ$ & $WZZ$ & $ZZZ$ \\
SM Cross Section (pb) & 0.000603400 & 0.000124200 & 0.000009634 & 0.000000972 \\
\hline
sm/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline 
Cwww/sm & 1.4 & 1.2 & 1.4 & 1.0 \\
\hline
Cw/sm & 1.1 & 1.1 & 1.2 & 1.1 \\
\hline 
Cb/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline

\hline
\hline
\end{tabular}
\end{center}
\label{tab:dim6scan}
\caption{Dimension 6 operators and their comparison to SM values for a 14~\TeV proton proton collider. This is for a coupling strength of $5^{-2}$ TeV. }
\end{table}

The dimension 8 operators have different unitarity bounds than the dimension 8 operators.  We have estimated these in the same way, with the same form factor tool avaliable with VBFNLO~\cite{unitarityCalculator}.  The bounds are shown for various values for Cwww in Figure~\ref{fig:unitaritydim6}.

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.5]{WWW_UnitarityBounddim6-eps-converted-to.pdf}
\caption{Unitarity bounds for the Cwww operator in various scenarios.}
\label{fig:unitarity}
\end{center}
\end{figure}

The statistical analysis is done in the same way as in Sec.~\ref{WWW}.  Figure~\ref{fig:cwwww} shows the $WWW$ templates used for the 14~\TeV machine, before the lepton invariant mass selection.  It is clear there is a large excess for this particular coupling value.  Figure~\ref{fig:unitaritysigdim6} shows the significance estimates for various Cwww values for 5 different hadron collider machines being studied for Snowmass and  Table~\ref{tab:WWWdim6} gives the approximate $5 \sigma$-significance discovery values. 

 Table~\ref{tab:WWW} gives the approximate $5 \sigma$-significance discovery values for the T0 operator for the 5 machines. 
\begin{table}[h]
\centering
\begin{tabular}{lccc} \hline 
                          &  $300\,\ifb$    & $1000\,\ifb$     & $3000\,\ifb$    \\
\hline $\sqrt(s) = 14$    &  8 TeV$^{-2}$ &        -           & 2.5 TeV$^{-2}$  \\
\hline $\sqrt(s) = 33$    &       -         &       -          & 2.0 TeV$^{-2}$   \\
\hline $\sqrt(s) = 100$   &       -         &  1.5 TeV$^{-2}$  & 1.0 TeV$^{-2}$  \\
\hline \hline \end{tabular}
\caption{Summary of expected sensitivity to anomalous $WWW$ production at various hadron collider machines, quoted in the terms of approximate $5 \sigma$-significance discovery values of $Cwww/\Lambda^2$.
}
\label{tab:WWWdim6}
\end{table}


\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.45]{WWW_33tevtemplate_dim6-eps-converted-to.pdf}
\caption{Invariant mass for $WWW$ at 33 TeV with the SM (blue) and $Cwww$ at $2~\TeV^{-2}$ (red).  }
\label{fig:cwwww}
\end{center}
\end{figure}



\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.95]{WWW_Significancedim6-eps-converted-to.pdf}
\caption{Significance values before unitarity (solid) and after unitarity cuts (dashed) for the $Cwww$ operator in various scenarios.}
\label{fig:unitaritysigdim6}
\end{center}
\end{figure}
%\newpage


==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = whitepaper

default: pdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
#	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

pdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
#	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 



==> WWZ.tex <==


\section{Cross-sections at the ILC, TLEP and CLIC}

In addition to the hadron colliders, we have also looked at cross-sections for the triboson processes $VVV$. The same dimension 8 model and final states discussed in Sec.~\ref{WWW} are considered.  However, because the collisions are electron-positron, only $WWZ$ results are reported.

\subsection{Monte Carlo Predictions}
The same Monte Carlo generation proceedure as described in Sec.~\ref{WWW} was followed again here, though for different collider settings.  The Madgraph~\cite{Alwall:2011uj} parameters were altered for e+ e- collisions and the polarization values expected at the different machines were also included.  Again, these follow the Snowmass recommendations~\cite{Avetisyan:2013sn1, Avetisyan:2013sn2}.

We performed a cross section scan to compare the SM cross sections to anomalous coupling cross sections for various coupling values and machine energies (Table~\ref{tab:dim8scanILC}).


\begin{table}[htdp]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Coupling & $ILC1$ & $TLEP1$ & $CLIC1$ & $CLIC2$ \\
SM Cross Section (pb) &  &  &  &  \\
\hline
sm/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline 
fm0/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
fm1/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
fm2/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
fm3/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
ft0/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
ft1/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
ft2/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline 

\hline
\hline
\end{tabular}
\end{center}
\label{tab:dim8scanILC}
\caption{Dimension 8 operators and their comparison to SM values. This is for a coupling strength of $10^{-4}$ TeV. }
\end{table}



==> bibtex.tex <==
%\renewcommand{\bibname}{\centerline{BIBLIOGRAPHY}}
%\unappendixtitle
%\newpage
%\phantomsection
%\addcontentsline{toc}{chapter}{BIBLIOGRAPHY}
\bibliography{bib}
%\bibliography{WWSupportNote}
%\bibliography{vv_fullyleptonic}


==> tribosons.tex <==
%\documentclass[11pt]{amsart}
%\usepackage{geometry}                % See geometry.pdf to learn the layout options. There are lots.
%\geometry{letterpaper}                   % ... or a4paper or a5paper or ... 
%\geometry{landscape}                % Activate for for rotated page geometry
%\usepackage[parfill]{parskip}    % Activate to begin paragraphs with an empty line rather than an indent
%\usepackage{graphicx}
%\usepackage{amssymb}
%\usepackage{epstopdf}
%\usepackage{feynmp}

%\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}
%\DeclareGraphicsRule{*}{mps}{*}{}
\section{Tribosons with aQGC in Effective Field Theory}
%\author{Jenny Holzbauer and Mandy Rominsky }
%\date{\today}                                           % Activate to display a given date or no date
%
%\begin{document}
%\maketitle

\subsection{Introduction}
In the Standard Model, the only allowed quartic couplings are $WWWW,  WWZZ,  WWZ  \gamma$ and $WW \gamma \gamma$  and they are completely specified. Measuring these couplings will provide stringent tests to the Standard model and help searches for physics beyond the standard model. The standard way to search for these couplings is to measure triboson production. $WWW$ production probes  $WWWW$, while $WWZ$ and $WW\gamma$ probe $WWZZ, WWZ \gamma$ and $WW\gamma \gamma$, respectively~\cite{theory}. This section focusses first on $WWW, WWZ, WZZ$ and $ZZZ$ with a  quick scan of the energies and cross sections, and then a case study from $WWW$ is highlighted with the promising operators. 

This analysis is carried out using effective Lagrangian theory~\cite{efftheory}. The details are explained in a separate document.  We tested both dimension 6 operators (list operators here) and dimension 8 operators. Since dim6 operators are sensitive to both triple and quartic gauge couplings, we found that these operators didn't show much sensitivity. However, dim8 is only sensitive to quartic gauge couplings and are therefore where we put our energy. 

\begin{figure}[htbp]
\begin{center}
\includegraphics{Feynmanwwzz.png}
\caption{Feynman diagrams from MadGraph~\cite{mg5} for the $WWZZ$ process. }
\label{fig:feynman}
\end{center}
\end{figure}

Figure~\ref{fig:feynman} shows example diagrams for the $WWZZ$ process. This Snowmass exercise was performed using MadGraph~\cite{mg5} for event generation, Pythia for showering,  a special version of Delphes~\cite{delphes} for the detector simulation and specially designed pile up files~\cite{pu}. 



\subsection{Effective theory with dimension 6 operators}

The dimension 6 operators that we looked at were $C_{W}$, $C_{WWW}$ and $C_{b}$. Table~\ref {tab:dim6scan} shows the cross section scan performed

\begin{table}[htdp]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\hline
Operator & $C_{W}$ & Coupling value & 5\\
\hline
Process & machine & energy & XSection \\
\hline
$WWZ$ & LHC & 14 TeV & number \\
\hline
$WWW$ & LHC & 14 TeV & number \\
\hline
$WZZ$ &LHC & 14 TeV & number \\
\hline
Operator & $C_{WWW}$ & Coupling value & 5\\
\hline 
Operator & $C_{b}$ & Coupling value & 5\\
\hline
\end{tabular}
\end{center}
\label{tab:dim6scan}
\caption{Dimension 6 operators}
\end{table}%



The $C_{W}$ operator was studied first.  All processes studied were decayed fully leptonically. Figure~\ref{fig:dim6scan} hows the number of events versus machine energy  for each of the three processes with the SM )$C_{W}$ set to 0) and the $C_{W}$ operator set to a value of 5. The $WZZ$ anomalous coupling shows a distinct difference between the SM shape and anomalous coupling, but between backgrounds and the low event rate, this is not a very promising channel. Figure~\ref{fig:cw1} shows the invariant mass of five leptons for 2 different machine energies, with 50,000 events, and requiring  all five leptons. 

\begin{figure}[htbp]
\begin{center}
\includegraphics{dim6scan.png}
\caption{Number of Events for different machine energies with the $C_W$ operator set to 5 and set to 0, which is the Standard Model case.}
\label{fig:dim6scan}
\end{center}
\end{figure}


\begin{figure}[htbp]
\begin{center}
\includegraphics{cw1.png}
\caption{Invariant mass of the 5 leptons in the $WZZ$ channel in the SM case (blue) and with $C_W$ turned on (red).. There are 50,000 events in the sample and a cut  requiring exactly 5leptons.  Background is not included in this plot. }
\label{fig:cw1}
\end{center}
\end{figure}



The $WWZ$ processes has more background when requiring four leptons, as compared to $WZZ$, but the signal rate is also expected to be higher. Figure~\ref{fig:cwwwz} shows the invariant mass for this process when requiring 4 leptons for two different machine energies. 

\begin{figure}[htbp]
\begin{center}
\includegraphics{cwwwz.png}
\caption{$WWZ$ process with SM (blue) and $C_W$, 50,000 events and requiring 4 leptons.}
\label{fig:cwwwz}
\end{center}
\end{figure}

Finally, the $WWW$ process has the largest cross section for the anomalous coupling, but it also will have more trouble with backgrounds~\ref{fig:cwwww}. 


\begin{figure}[htbp]
\begin{center}
\includegraphics{cwwww.png}
\caption{Invariant mass for $WWW$ at 13 TeV with the SM (blue) and $C_W$ (red).  }
\label{fig:cwwww}
\end{center}
\end{figure}



In addition to testing $C_{W}$, the $C_{WWW}$ and $C_b$ operators were probed. The $C_b$ operator showed no sensitivity to anomalous couplings, but the $C_{WWW}$ operator shows a larger sensitivity than $C_{W}$~\ref{fig:cw3w3}.


\begin{figure}[htbp]
\begin{center}
\includegraphics{cw3w3.png}
\caption{The $WWW$ invariant mass with the SM (blue) and $C_{WWW}$ operator set to 5. }
\label{fig:cw3w3}
\end{center}
\end{figure}


While some of the dimension 6 operators showed reasonable sensitivity to anomalous couplings, we decided to focus on the dimension 8 operators because they are more sensitive to the quartic couplings. 


\subsection{Effective Theory operators dimension 8}

Dimension 8 operators are only sensitive to quartic gauge couplings and offer a good way to explore anomalous couplings.  The dimension 8 operators sensitive to $WWW, WWZ, WZZ$  and $ ZZZ$ are listed in Table~\ref{tab:dim8} . 


\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
 & $WWWW$ & $WWZZ$ & $ZZZZ$ \\
 \hline
 $\mathcal{L}_{S,0}$ , $\mathcal{L}_{S,1}$ &$X$ & $X$&$X$ \\
 \hline 
 $\mathcal{L}_{M,0}$ , $\mathcal{L}_{M,1}$ ,$\mathcal{L}_{M,6}$ , $\mathcal{L}_{M,7}$ &$X$ & $X$&$X$ \\
 \hline 
$\mathcal{L}_{M,2}$ , $\mathcal{L}_{M,3}$ ,$\mathcal{L}_{M,4}$ , $\mathcal{L}_{M,5}$ &$O$ & $X$&$X$ \\
 \hline 
$\mathcal{L}_{T,0}$ , $\mathcal{L}_{T,1}$ ,$\mathcal{L}_{T,3}$ &$X$ & $X$&$X$ \\
 \hline 
 $\mathcal{L}_{T,5}$ , $\mathcal{L}_{T,6}$ ,$\mathcal{L}_{T,7}$ &$O$ & $X$&$X$ \\
 \hline 
 $\mathcal{L}_{T,8}$ , $\mathcal{L}_{T,9}$ &$O$ & $O$&$X$ \\
 \hline 
 \hline
 
\end{tabular}
\end{center}
\label{tab:dim8}
\end{table}%



An extensive cross section scan was performed to compare the SM cross sections to anomalous coupling cross sections for various coupling values and machine energies (Table~\ref{tab:dim8scan}). From the study, the T0 operator was found to be the most sensitive to anomalous couplings, particularly in the $WWW$ channel. 


\begin{table}[htdp]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Coupling & $WWW$ & $WWZ$ & $WZZ$ & $ZZZ$ \\
SM Cross Section (pb) & 0.000568000 & 0.000111800 & 0.000009634 & 0.000000972 \\
\hline
sm/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline 
fs0/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline
fs1/sm & 1.0 & 1.0 & 1.0 & 1.0 \\
\hline 
fm0/sm & 1.49 & 1.09 & 1.05 & 1.02 \\
\hline
fm1/sm & 1.18 & 1.02 & 1.04 & 1.03 \\
\hline
fm2/sm & 1.0 & 1.05 & 1.0 & 1.02 \\
\hline
fm3/sm & 1.0 & 1.01 & 1.00 & 1.01 \\
\hline
ft0/sm & 19.10 & 4.23 & 3.38 & 2.90\\
\hline
ft1/sm & 15.88 & 2.23 & 2.83 & 2.90 \\
\hline
ft2/sm & 4.61 & 1.33 & 1.35 & 1.54 \\
\hline
ft8/sm & 1.0 & 1.0 & 1.0 & 1.31 \\
\hline
ft9/sm & 1.0 & 1.0 & 1.0 & 1.08 \\
\hline 

\hline
\hline
\end{tabular}
\end{center}
\label{tab:dim8scan}
\caption{Dimension 8 operators and their comparison to SM values. This is for a coupling strength of $10^{-4}$ TeV. }
\end{table}%

\subsection{$WWW$ case study}
The $WWW$ was chosen for further study. The main background for the $WWW$ anomalous coupling is SM $WWW$, followed by  dibosons ($WW,WZ, ZZ$), z+jets, z+photon, w+2jets and ttbar dilepton.  With the except of the ttbar background, the other backgrounds are eliminated  by using lepton charge and number of leptons cuts. The ttbar background is handled by making a cut on the log of the invariant mass of the 3 leptons to be less than 3.1. 

To make this a more realistic study, pile up was added according to the Snowmass scheme~\cite{pu}.  The significance was calculated using a LLR calculation and Frequentist approach~\cite{sigcalc}. As can be seen in Figures~ref{fig:t0www14} and ~\ref{fig:t0www33}. 


\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.25]{14TeVplot-eps-converted-to.pdf}
\caption{$WWW$ invariant mass with pileup added and backgrounds reduced. The SM is in blue and the mass with $T0$ turned on is in blue.}
\label{fig:t0www14}
\end{center}
\end{figure}



\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.25]{33TeVplot-eps-converted-to.pdf}
\caption{$WWW$ invariant mass with pileup added and backgrounds reduced. The SM is in blue and the mass with $T0$ turned on is in blue.}
\label{fig:t0www33}
\end{center}
\end{figure}


We found that some of the events in the analysis violate unitarity. After taking this into account our significances have change. Figure~\ref{fig:unitaritysig} shows how the significance in a variety of scenarios changes when unitarity bounds are applied. 

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.5]{sigplot2-eps-converted-to.pdf}
\caption{Significance values before unitarity (solid) and after unitarity cuts (dashed) for the $T0$ operator in various scenarios.}
\label{fig:unitaritysig}
\end{center}
\end{figure}
\newpage

\subsection{Other Studies}
Besides LHC scenarios, the lepton collider scenarios were studied. Future versions of this document will include the ILC scenario table. 





%\newpage
%\begin{thebibliography}{1}
%\bibitem{theory} "Vector Boson Fusion and Quartic Boson Couplings", D. Green, arXiv:hep-ph/0306160, 2003
%\bibitem{efftheory} "Effective Field Theory: A modern approach to anomalous couplings", Celine Degrande, Nicolas Greiner, Wolfgang Kilian, Olivier Mattelaer, Harrison Mebane, Tim Stelzer, Scott Willenbrock, Cen Zhang, arXiv:1205.4231 [hep-ph], 2012
%\bibitem{mg5} MadGraph5: http://madgraph.phys.ucl.ac.be
%\bibitem{delphes} "Snowmass Energy Frontier Simulations for Hadron Colliders", A. Avetisyan et. al. arXiv:1307.XXX, July 2013
%\bibitem{pu} "Standard Model Background Generation for Snowmass using Madgraph", A. Avetisyan et. al. arXiv:1307.XXX, July 2013
%\bibitem{sigcalc} Private calculation program, will need a better reference. 
%\end{thebibliography}



  

%\subsection{}



%\end{document}  

